Correlated Random Measures

We develop correlated random measures, random measures where the atom weights can exhibit a flexible pattern of dependence, and use them to develop powerful hierarchical Bayesian nonparametric models. Hierarchical Bayesian nonparametric models are usually built from completely random measures, a Poisson-process based construction in which the atom weights are independent. Completely random measures imply strong independence assumptions in the corresponding hierarchical model, and these assumptions are often misplaced in real-world settings. Correlated random measures address this limitation. They model correlation within the measure by using a Gaussian process in concert with the Poisson process. With correlated random measures, for example, we can develop a latent feature model for which we can infer both the properties of the latent features and their dependency pattern. We develop several other examples as well. We study a correlated random measure model of pairwise count data. We derive an efficient variational inference algorithm and show improved predictive performance on large data sets of documents, web clicks, and electronic health records.

==> preamble.tex <==
 \pdfminorversion=4

\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.25ex\@plus -1ex \@minus -.2ex}%
                                   {.3ex \@plus.2ex}%
                                   {\centering\large %
                                    \scshape\bfseries\uppercase}}

\usepackage{titlesec}
\titlelabel{\thetitle.\quad}


%\renewcommand{\section}{\@startsection {section}{1}{\z@}%
%             {-3.5ex \@plus -1ex \@minus -.2ex}%
%             {.3ex \@plus .2ex}%
%             {\centering\normalfont\scshape\bfseries}}

% ##### FONTS

\renewcommand{\rmdefault}{ptm}
\usepackage{amssymb}
%\usepackage[amssymbols,subscriptcorrection,slantedGreek,nofontinfo,mtpcal,mtpbb]{mtpro2}
\usepackage[T1]{fontenc}


% ##### MATH

\usepackage{amsmath, amsthm, amsfonts}
\usepackage{mathtools}

% ##### FIGURES

\usepackage{graphicx}
\usepackage{pdflscape}

% ##### BIBLIOGRAPHY AND REFERENCE

\usepackage{natbib}
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=MidnightBlue}
\hypersetup{linkcolor=Black}

\usepackage[
  paper  = letterpaper,
  left   = 1in,
  right  = 1in,
  top    = 1.0in,
  bottom = 1.0in,
  ]{geometry}


% ##### ALGORITHMS

\usepackage[algoruled]{algorithm2e}
\usepackage{algorithmic}

% ##### COLOR

\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}
\definecolor{shadecolor}{gray}{0.9}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\E}{\textrm{E}}
\newcommand{\corr}{\textrm{CorrRM}}
\newcommand{\myeqp}[1]{Eq.\ref{eq:#1}}
\newcommand{\mysec}[1]{Section~\ref{sec:#1}}
\newcommand{\myfig}[1]{Figure~\ref{fig:#1}}
\newcommand{\myappendix}[1]{Appendix \ref{appendix:#1}}
\newcommand{\edist} {\,{\buildrel d \over =}\,}
\newcommand{\gammapro}{\textrm{Gamma-Process}}
\newcommand{\gaussianpro}{\textrm{Gaussian-Process}}
\newcommand{\poissonpro}{\textrm{Poisson-Process}}
\newcommand{\p}{\noindent \P \, \, }
\newcommand{\bbR}{\mathbb{R}}
\newtheorem{proposition}{Proposition}
\newcommand{\g}{\, | \,}
\newcommand{\myeq}[1]{Equation~\ref{eq:#1}}
\newcommand{\parhead}[1]{\paragraph{#1}}



